Local Read-Write Operations in Sensor Networks

Designing protocols and formulating convenient programming units of abstraction for sensor networks is challenging due to communication errors and platform constraints. This paper investigates properties and implementation reliability for a \emph{local read-write} abstraction. Local read-write is inspired by the class of read-modify-write operations defined for shared-memory multiprocessor architectures. The class of read-modify-write operations is important in solving consensus and related synchronization problems for concurrency control. Local read-write is shown to be an atomic abstraction for synchronizing neighborhood states in sensor networks. The paper compares local read-write to similar lightweight operations in wireless sensor networks, such as read-all, write-all, and a transaction-based abstraction: for some optimistic scenarios, local read-write is a more efficient neighborhood operation. A partial implementation is described, which shows that three outcomes characterize operation response: success, failure, and cancel. A failure response indicates possible inconsistency for the operation result, which is the result of a timeout event at the operation's initiator. The paper presents experimental results on operation performance with different timeout values and situations of no contention, with some tests also on various neighborhood sizes.

==> pst-bar.tex <==
\csname PSTBarLoaded\endcsname%
\let\PSTBarLoaded\endinput%
\ifx\PSTplotLoaded\endinput\else\input pst-plot.tex\fi%
\pstheader{pst-bar.pro}%
\input pst-key.tex%

\def\fileversion{0.7a}
\def\filedate{2004/09/24}
\message{`pst-bar' v\fileversion, \filedate\space (Alan Ristow)}%

\define@key{psset}{barsep}{\edef\psk@barsep{#1}}%
\define@key{psset}{barcolsep}{\edef\psk@barcolsep{#1}}%
\define@key{psset}{barstyle}{\edef\psk@barstyle{#1}}%
\define@key{psset}{barlabelrot}{\edef\psk@barlabelrot{#1}}%
\setkeys{psset}{barsep=0.0,barcolsep=0.4,barstyle=\@empty,barlabelrot=0}%
%
% chartstyle=cluster|stack|block  (0,1,2)
\def\psset@chartstyle#1{\pst@expandafter\psset@@chartstyle{#1}\@nil\psk@chartstyle}
\def\psset@@chartstyle#1#2\@nil#3{%
  \ifx#1c\let#3\z@\else
    \ifx#1s\let#3\@ne\else
      \ifx#1b\let#3\tw@\else
        \@pstrickserr{Bad argument: `#1#2'}\@ehpa
      \fi
    \fi
  \fi
}%
\psset@chartstyle{cluster}%
%
% orientation=vertical|horizontal (0,1)
\def\psset@orientation#1{\pst@expandafter\psset@@orientation{#1}\@nil\psk@orientation}
\def\psset@@orientation#1#2\@nil#3{%
  \ifx#1h\let#3\p@\else
    \ifx#1v\let#3\z@\else
      \@pstrickserr{Bad argument: `#1#2'}\@ehpa
    \fi
  \fi
}%
\psset@orientation{vertical}%

\def\psset@header#1{%
  \pst@expandafter\psset@@header{#1}\@nil\psk@header
}%
\def\psset@@header#1#2\@nil#3{%
  \ifx#1t\let#3\z@\else
    \ifx#1f\let#3\@ne\else
      \@pstrickserr{Bad argument: `#1#2'}\@ehpa
    \fi
  \fi
}%
\psset@header{true}%

\def\psbarchart{\def\pst@par{}\pst@object{psbarchart}}%
\def\pstbar@header{\@empty}%
\def\psbarlabel#1{#1}%
\def\psbarlabelsep{0pt}%
\def\psbarscale(#1)#2{%
  \def\psbar@mul{#1\space}%
  \def\psbar@psop{#2\space}%
}
\def\psbar@mul{1\space}%
\def\psbar@psop{\@empty}%

\newread\pstbar@file%

% Define bar chart styles

\def\psset@barstyle#1{\def\@barstylelist{#1}}%
\def\newpsbarstyle#1#2{\@namedef{psbarcs@#1}{\psset{#2}}}%

\def\begin@barstyle{\def\pst@tempd{/barstyles [ }}%
\def\add@barstyle{%
  \def\pst@code{}%
  \ifpsshadow%
    \pst@closedshadow%
  \fi%
  \ifdim\psk@border\p@>\z@%
    \pst@addborder%
  \fi%
  \psk@fillstyle%
  \pst@stroke%
  \ifpsdoubleline%
    \pst@doublestroke%
  \fi%
  \def\pst@tempa{\strip@pt\psk@orientation}%
  \edef\pst@tempd{ \pst@tempd (%
    \pst@tempc \psk@cornersize%
    xbar1 ybar1 xbar2 ybar2 4 -\pst@tempa\space roll
    \psk@dimen%
    \tx@Frame%
    \pst@code )%
  }%
}
\def\end@barstyle{\edef\pst@tempd{ \pst@tempd ] def }}%

\def\setbarstyle{%
  \begin@barstyle%
  \expandafter\@setbarstyle\@barstylelist,\@nil\ignorespaces%
  \end@barstyle%
}%
\def\@setbarstyle#1,{%
  \@@setbarstyle{#1}%
  \@ifnextchar\@nil{\@gobble}{\@setbarstyle}%
}%
\def\@@setbarstyle#1{%
  \@ifundefined{psbarcs@#1}%
  {\@pstrickserr{Custom bar chart style `#1' undefined}\@ehpa}%
  {\@nameuse{psbarcs@#1}\add@barstyle}%
}%

% Default bar chart styles

\newpsbarstyle{red}{fillcolor=red,fillstyle=solid,framearc=0}%
\newpsbarstyle{green}{fillcolor=green,fillstyle=solid,framearc=0}%
\newpsbarstyle{blue}{fillcolor=blue,fillstyle=solid,framearc=0}%
\newpsbarstyle{black}{fillcolor=black,fillstyle=solid,framearc=0}%
\newpsbarstyle{white}{fillcolor=white,fillstyle=solid,framearc=0}%
\newpsbarstyle{gray}{fillcolor=gray,fillstyle=solid,framearc=0}%
\newpsbarstyle{lightgray}{fillcolor=lightgray,fillstyle=solid,framearc=0}%
\newpsbarstyle{darkgray}{fillcolor=darkgray,fillstyle=solid,framearc=0}%

\psset@barstyle{black,darkgray,gray,lightgray,white,red,green,blue}%

\def\readpsbardata{\@ifnextchar[{\readpsbardata@i}{\readpsbardata@i[]}}

\def\readpsbardata@i[#1]#2#3{%
  \def\pst@tempa{#1}%
  \ifx\pst@tempa\@empty\else\psset{#1}\fi
  \openin\pstbar@file=#3\relax%
  \ifeof\pstbar@file%
    \@pstrickserr{Data file `#3' not found.}\@ehpa
  \else
    \def\pst@tempb{\@empty}%
    \ifx\psk@header\z@%
      \@readpsbarheader%
    \fi
    \readpsbardata@ii%
    \edef\pst@tempb{[\pst@tempb]}%
    \let#2\pst@tempb%
  \fi
  \closein\pstbar@file%
}%

\def\readpsbardata@ii{%
  \read\pstbar@file to \pst@tempa
  \ifeof\pstbar@file
    \relax
  \else
    \edef\pst@tempb{\pst@tempb [}%
    \expandafter\readpsbardata@iii\pst@tempa,\@nil\ignorespaces%
    \edef\pst@tempb{\pst@tempb ]}%
    \readpsbardata@ii%
  \fi
}%

\def\readpsbardata@iii#1,{%
  \edef\pst@tempb{\pst@tempb #1\space}%
  \@ifnextchar\@nil{\@gobble}{\readpsbardata@iii}%
}%

\def\@readpsbarheader{%
  \read\pstbar@file to \pst@tempa
  \ifeof\pstbar@file
    \relax
  \else
    \let\pstbar@header\pst@tempa
  \fi
}%

% Apply labels from file header to bar chart columns.
% TODO: Deal with column headings that contain commas.

% The trimspaces command is (c) Michael Downes 1994
% (http://www.tug.org/tex-archive/info/aro-bend/answer.015).
\catcode`\Q=3
\def\psbar@trimspaces#1{%
  \begingroup
  \aftergroup\toks\aftergroup0\aftergroup{%
  \expandafter\trimb\expandafter\noexpand#1Q Q}%
  \edef#1{\the\toks0}%
}
\def\trimb#1 Q{\trimc#1Q}
\def\trimc#1Q#2{\afterassignment\endgroup \vfuzz\the\vfuzz#1}
\catcode`\Q=11

\def\pstbar@xlabels{%
  \pst@dima=-0.5pt\relax%
  \expandafter\pstbar@xlabels@i\pstbar@header,\@nil\ignorespaces%
}%

\def\pstbar@xlabels@i#1,{%
  \def\pst@tempa{#1}%
  \psbar@trimspaces\pst@tempa%
  \advance\pst@dima by 1pt%
  \def\pst@tempb{\strip@pt\pst@dima}%
  \uput[-90]{\psk@barlabelrot}(\pst@tempb,-\psbarlabelsep){\psbarlabel{\pst@tempa}}%
  \@ifnextchar\@nil{\@gobble}{\pstbar@xlabels@i}%
}%

\def\pstbar@labelcount#1{%
  \pst@dima=0pt\relax%
  \expandafter\pstbar@labelcount@i\pstbar@header,\@nil\ignorespaces%
  \let#1\pst@dima%
}%

\def\pstbar@labelcount@i#1,{%
  \advance\pst@dima by 1pt%
  \@ifnextchar\@nil{\@gobble}{\pstbar@labelcount@i}%
}%

\def\pstbar@ylabels{%
  \pstbar@labelcount{\pst@dima}%
  \advance\pst@dima by 0.5pt%
  \expandafter\pstbar@ylabels@i\pstbar@header,\@nil\ignorespaces%
}%

\def\pstbar@ylabels@i#1,{%
  \def\pst@tempa{#1}%
  \psbar@trimspaces\pst@tempa%
  \advance\pst@dima by -1pt%
  \def\pst@tempb{\strip@pt\pst@dima}%
  \uput[180]{\psk@barlabelrot}(-\psbarlabelsep,\pst@tempb){\psbarlabel{\pst@tempa}}%
  \@ifnextchar\@nil{\@gobble}{\pstbar@ylabels@i}%
}%

\def\psbarchart@i#1{%
  \pst@killglue%
  \begingroup%
    \use@par%
    \psbarchart@ii{#1}%
  \endgroup%
  \ignorespaces%
}%

\def\psbarchart@ii#1{%
  \begin@SpecialObj%

    % Save contents of \pst@code and load start-of-path code
    % into \pst@tempc

    \let\pst@tempb\pst@code%
    \def\pst@code{}%
    \solid@star%
    \let\pst@tempc\pst@code%

    % Load end-of-path code into \pst@tempd and restore original
    % contents of \pst@code

    \begin@barstyle%
    \expandafter\@setbarstyle\@barstylelist,\@nil\ignorespaces%
    \end@barstyle%
    \let\pst@code\pst@tempb%

    % Draw bar chart

    \pst@checknum\psk@barcolsep\pst@tempa%
    \pst@checknum\psk@barsep\pst@tempb%
    \ifx\psk@orientation\z@             % vertical
      \pst@dima=\psxunit%
      \pst@dimb=\psyunit%
      \def\pst@tempc{true}%
    \else\ifx\psk@orientation\p@        % horizontal
      \pst@dima=\psyunit%
      \pst@dimb=\psxunit%
      \def\pst@tempc{false}%
    \else
      \@pstrickserr{Bad orientation specification}\@ehpa
    \fi\fi
    \ifcase\psk@chartstyle% chartstyle=cluster
      \addto@pscode{%
        \pst@tempd%
        /BARDATA #1 def
        /nbars BARDATA length def
        /ncols BARDATA 0 get length def
        /colwidth \pst@number\pst@dima def
        /barcolsep \pst@tempa \pst@number\pst@dima mul def
        /barsep \pst@tempb \pst@number\pst@dima mul def
        /barwidth colwidth barcolsep sub nbars 1 sub barsep mul sub nbars div def
        /bXoffset 0.5 barcolsep mul def
        /colcount \pst@tempc\space {0}{ncols 1 sub} ifelse def
        /barcount 0 def
        /ybar1 0 def
        BARDATA {
          /DATAVECTOR exch def
          DATAVECTOR {
            /ybar2 exch \psbar@psop \psbar@mul mul \pst@number\pst@dimb mul def
            /xoffset barwidth barsep add barcount mul bXoffset add def
            /xbar1 colcount colwidth mul xoffset add def
            /xbar2 xbar1 barwidth add def
            ybar1 ybar2 ne {  % if ybar1 == ybar2, don't stroke a path
              newpath
              barstyles barcount get cvx exec
            } if
            /colcount \pst@tempc\space {colcount 1 add}{colcount 1 sub} ifelse def
          } forall
          /colcount \pst@tempc\space {0}{ncols 1 sub} ifelse def
          /barcount barcount 1 add def
        } forall
      }%
    \or%  chartstyle=stack
      \addto@pscode{%
        \pst@tempd%
        tx@BarDict begin
        /BARDATA #1 transpose def
        /ncols BARDATA length def
        /colwidth \pst@number\pst@dima def
        /barcolsep \pst@tempa \pst@number\pst@dima mul def
        /barwidth colwidth barcolsep sub def
        /bXoffset 0.5 barcolsep mul def
        /colcount \pst@tempc\space {0}{ncols 1 sub} ifelse def
        /barcount 0 def
        /ybar1 0 def
        BARDATA {
          /DATAVECTOR exch def
          /xbar1 colcount colwidth mul bXoffset add def
          /xbar2 xbar1 barwidth add def
          DATAVECTOR {
            /ybar2 exch \psbar@psop \psbar@mul mul \pst@number\pst@dimb mul ybar1 add def
            ybar1 ybar2 ne {  % if ybar1 == ybar2, don't stroke a path
              newpath
              barstyles barcount get cvx exec
              closepath
            } if
            /ybar1 ybar2 def
            /barcount barcount 1 add def
          } forall
          /barcount 0 def
          /ybar1 0 def
          /colcount \pst@tempc\space {colcount 1 add}{colcount 1 sub} ifelse def
        } forall
        end
      }%
    \or% chartstyle=block
      \addto@pscode{%
        \pst@tempd%
        tx@BarDict begin
        /BARDATA #1 transpose def
        /ncols BARDATA length def
        /nbars BARDATA 0 get length 2 idiv def
        /colwidth \pst@number\pst@dima def
        /barcolsep \pst@tempa \pst@number\pst@dima mul def
        /barsep \pst@tempb \pst@number\pst@dima mul def
        /barwidth colwidth barcolsep sub nbars 1 sub barsep mul sub nbars div def
        /bXoffset 0.5 barcolsep mul def
        /colcount \pst@tempc\space {0}{ncols 1 sub} ifelse def
        /barcount 0 def
        /ybar1 0 def
        BARDATA {
          /DATAVECTOR exch def
          0 1 nbars 1 sub {
            dup
            /ybar1 exch 2 mul DATAVECTOR exch get \psbar@psop \psbar@mul mul \pst@number\pst@dimb mul def
            /ybar2 exch 2 mul 1 add DATAVECTOR exch get \psbar@psop \psbar@mul mul \pst@number\pst@dimb mul def
            /xoffset barwidth barsep add barcount mul bXoffset add def
            /xbar1 colcount colwidth mul xoffset add def
            /xbar2 xbar1 barwidth add def
            ybar1 ybar2 ne {  % if ybar1 == ybar2, don't stroke a path
              newpath
              barstyles barcount get cvx exec
            } if
            /barcount barcount 1 add def
          } for
          /barcount 0 def
          /colcount \pst@tempc\space {colcount 1 add}{colcount 1 sub} ifelse def
        } forall
        end
      }%
    \else%
      \@pstrickserr{Unknown chart style.}\@ehpa%
    \fi%
    \ifx\psk@orientation\z@%
      \pstbar@xlabels%
    \else
      \pstbar@ylabels%
    \fi
  \end@SpecialObj%
}%

\endinput

\iffalse
%% CHANGE-LOG
 v 0.7a   2004/09/24
    Removed some debugging code that was accidentally left in the last release.
    The removed code was harmless, but caused confusion for some users.

 v 0.7    2004/09/15
    Made a minor change to \psbarscale so its functionality would be more
    closely analogous to the \pstScale command from the pstricks-add pacakge.
    Improved documentation. Set default barstyle to list of all available
    barstyles. First release to CTAN.

 v 0.6    2004/09/09
    Added orientation parameter and horizontal bar-drawing capability. Removed
    erroneous correction factor for linewidth from stacked bar chart.

 v 0.5    2004/09/02
    Added header parameter for \readpsbardata. Improved handling of headers in
    the data file -- spaces may now be included in a header item, though commas
    still may not.

 v 0.4    2004/08/29
    Added "block" chartstyle. Updated \readpsbardata to use .csv for both
    header and data. Introduced \psbarscale command. First release to pstricks
    mailing list, 2004/09/01.

 v 0.3    2004/08/26
    Added command \readpsbardata to read data for bar chart directly from a
    .csv file with the first row containing the column labels.

 v 0.2a   2004/08/23
    Changed colsep parameter name to barcolsep to avoid clash with psmatrix.

 v 0.2    2004/08/22
    Added stacked bar chart, chartstyle parameter, and introduced pst-bar.pro
    prologue with transpose command.

 v 0.1    2004/08/21
    Clustered bar chart.
\fi

